ChartInstruct: Instruction Tuning for Chart Comprehension and Reasoning

Charts provide visual representations of data and are widely used for analyzing information, addressing queries, and conveying insights to others. Various chart-related downstream tasks have emerged recently, such as question-answering and summarization. A common strategy to solve these tasks is to fine-tune various models originally trained on vision tasks language. However, such task-specific models are not capable of solving a wide range of chart-related tasks, constraining their real-world applicability. To overcome these challenges, we introduce ChartInstruct: a novel chart-specific vision-language Instruction-following dataset comprising 191K instructions generated with 71K charts. We then present two distinct systems for instruction tuning on such datasets: (1) an end-to-end model that connects a vision encoder for chart understanding with a LLM; and (2) a pipeline model that employs a two-step approach to extract chart data tables and input them into the LLM. In experiments on four downstream tasks, we first show the effectiveness of our model--achieving a new set of state-of-the-art results. Further evaluation shows that our instruction-tuning approach supports a wide array of real-world chart comprehension and reasoning scenarios, thereby expanding the scope and applicability of our models to new kinds of tasks.

==> Novel_task_samples.tex <==
\begin{table}[t]
 \setlength\extrarowheight{1pt}
 \centering

 
 \scalebox{0.74s}{\begin{tabular}{l|c}
  
  \toprule
  
  \multirow{1}{*}{\textbf{Task Group}} & \multirow{1}{*}{\textbf{\#Examples}} \\
\midrule
Pattern and Outlier Detection & 16,977 \\
  Statistical Analysis & 9,148 \\
  Extremum Identification & 6,545\\
  Item Correlations & 6,142 \\
  General Comparison & 4,709\\
  Relative Change Calculation & 4,108\\
  Time Series and Future Value Prediction & 1,944 \\
  Data Point Identification & 1,670\\
  Performance and Result Analysis & 1,396\\
  Data Categorization & 533\\
  Distribution analysis & 280\\
  \bottomrule
  

  
 
 \end{tabular}}
 \caption{\small {The number of generated examples for various groups of new tasks created by GPT-4.
 }
 \vspace{-3mm}
 }
 \label{tab:NovelCounts}
\end{table}




==> Task_chart_count.tex <==
\begin{table*}[t]
 \setlength\extrarowheight{1pt}
 \centering
 
 
 \scalebox{0.67}{\begin{tabular}{lcccccc|c}
  
  \toprule
  
  \multirow{1}{*}{Dataset
  } & \multirow{1}{*}{CoT Reasoning} & \multicolumn{1}{c}{Chart Summarization} & 
   \multicolumn{1}{c}{Fact Checking} & \multicolumn{1}{c}{Open-ended QA} &
   \multicolumn{1}{c}{Coding Abilities}& \multicolumn{1}{c}{Novel Tasks} 
 \multicolumn{1}{c}{ Distinct Charts}\\
                                             
  
  \midrule

  Statista   & 736 & 4,159 & 2,047 
  &1,485  & 400 & - &  9,992\\ 

  PlotQA   & 703 & 3977 & 1002 
  & 3966 &  400 & - &  8,199\\

  OECD/OWID   &722 & 3999   
  & 2016 & 3961  & 500 & -&  10,949\\

  WebCrawled   & 2,433 & 41,741 & 2,500 
  & 2,448  & 2,390 & 2,606 &  41,742\\
  \midrule
  Total  & 4,594 & 53,876 & 7,565 & 11,860  & 3,690 & 2,606 & 70,882
  \\ \bottomrule
  
 
 \end{tabular}}
 \vspace{-3mm}
 \caption{\small {breakdown of Distinct charts appearing on different tasks. Some of them appear in more than one task, counting in the total.\mehrad{Table Added. Do we want to marge with table 2?}
 }
 \vspace{-3mm}
 }
 \label{tab:chart_count}
\end{table*}



